Leading Isospin Breaking effects in nucleon and $\Delta$ masses

We present a lattice calculation of the leading corrections to the masses of nucleons and $\Delta$ resonances. These are obtained in QCD+QED at $1$st order in the Isospin Breaking parameters $\alpha_{EM}$, the electromagnetic coupling, and $\frac{{\hat{m}}_d - {\hat{m}}_u}{\Lambda_{QCD}}$, coming from the mass difference between $u$ and $d$ quarks.

==> Makefile <==
CC = pdflatex
TEX = main.tex
PDF = main.pdf
BCF = main.bcf
BIB = biblio.bib

show: $(PDF) $(TEX)
	evince $(PDF) &

$(BCF): $(BIB) $(TEX)
	make -B $(PDF)
	biber $(BCF)
	make -B $(PDF)
	make -B $(PDF)	

$(PDF): $(TEX)
	$(CC) $(TEX)

all: $(BCF)
	make clean

# 
# dt = 1s # time between subsequent compilations 
# automatic:
# 	clear
# 	echo "X" | make all & # in case of errors
# 	sleep $(dt) # time separation between compilations
# 	make automatic # recursive call to this target
# 
# 

clean:
	@rm *~ *.gz *.fls *.fdb_latexmk *.log *.aux *.xml \
	*.bbl *.blg *.out diagram.* *.bcf *.mp  \
	2> /dev/null || true
	


==> QCDQED/Data/TeX/amus/values.tex <==
\begin{tabular}{l|c|c}
$\beta$  &  $a m_{s_1}^{(0)}$ &  $a m_{s_2}^{(0)}$ \\ 
\hline \\[-2.0ex] 
1.90 & 0.0242 & 0.0261 \\ 
1.95 & 0.0216 & 0.0230 \\ 
2.10 & 0.0176 & 0.0186 \\ 
\end{tabular}


==> isoQCD/Data/TeX/amus/values.tex <==
\begin{tabular}{l|c|c|c}
$\beta$  &  $a m_{s_1}$ &  $a m_{s_2}$ &  $a m_{s_3}$ \\ 
\hline \\[-2.0ex] 
1.90 & 0.0220 & 0.0260 & 0.0300 \\ 
1.95 & 0.0190 & 0.0220 & 0.0250 \\ 
2.10 & 0.0136 & 0.0161 & 0.0186 \\ 
\end{tabular}


==> isoQCD/Data/TeX/ensembles/masses/K_Omega.tex <==
\begin{tabular}{l|c|c}
Ensemble & $M_K$ (MeV) & $M_\Omega$ (GeV) \\ 
\hline \\[-2.0ex] 
A100.24	& $547.3(5.5)$ $\,\,$ $580.5(5.8)$ $\,\,$ $612.0(6.1)$ $\,\,$  & $1.673(15)$ $\,\,$ $1.732(16)$ $\,\,$ $1.789(17)$ $\,\,$  \\ 
A30.32	& $484.4(5.2)$ $\,\,$ $521.1(5.6)$ $\,\,$ $555.6(6.0)$ $\,\,$  & $1.623(15)$ $\,\,$ $1.683(16)$ $\,\,$ $1.742(16)$ $\,\,$  \\ 
A40.20	& $500.7(5.7)$ $\,\,$ $536.8(6.0)$ $\,\,$ $570.7(6.3)$ $\,\,$  & $1.663(25)$ $\,\,$ $1.714(24)$ $\,\,$ $1.765(23)$ $\,\,$  \\ 
A40.24	& $496.9(5.4)$ $\,\,$ $532.9(5.7)$ $\,\,$ $566.7(6.0)$ $\,\,$  & $1.647(21)$ $\,\,$ $1.705(21)$ $\,\,$ $1.761(22)$ $\,\,$  \\ 
A40.32	& $491.5(5.0)$ $\,\,$ $527.6(5.4)$ $\,\,$ $561.6(5.7)$ $\,\,$  & $1.628(17)$ $\,\,$ $1.688(17)$ $\,\,$ $1.747(18)$ $\,\,$  \\ 
A40.40	& $490.4(5.1)$ $\,\,$ $526.3(5.5)$ $\,\,$ $560.1(5.8)$ $\,\,$  & $1.635(16)$ $\,\,$ $1.696(17)$ $\,\,$ $1.756(17)$ $\,\,$  \\ 
A40.48	& $491.2(5.2)$ $\,\,$ $527.3(5.5)$ $\,\,$ $561.3(5.9)$ $\,\,$  & $1.638(19)$ $\,\,$ $1.699(19)$ $\,\,$ $1.757(19)$ $\,\,$  \\ 
A50.32	& $500.3(5.0)$ $\,\,$ $536.0(5.4)$ $\,\,$ $569.5(5.8)$ $\,\,$  & $1.635(17)$ $\,\,$ $1.697(17)$ $\,\,$ $1.756(18)$ $\,\,$  \\ 
A60.24	& $512.3(5.5)$ $\,\,$ $547.2(5.9)$ $\,\,$ $580.3(6.3)$ $\,\,$  & $1.639(24)$ $\,\,$ $1.700(24)$ $\,\,$ $1.759(23)$ $\,\,$  \\ 
A80.24	& $528.1(5.6)$ $\,\,$ $562.1(5.9)$ $\,\,$ $594.3(6.3)$ $\,\,$  & $1.647(19)$ $\,\,$ $1.709(19)$ $\,\,$ $1.769(19)$ $\,\,$  \\ 
\hline \\[-2.0ex] 
B25.32	& $473.9(4.8)$ $\,\,$ $505.4(5.1)$ $\,\,$ $535.0(5.4)$ $\,\,$  & $1.616(15)$ $\,\,$ $1.664(16)$ $\,\,$ $1.712(16)$ $\,\,$  \\ 
B35.32	& $483.0(4.9)$ $\,\,$ $513.9(5.2)$ $\,\,$ $543.2(5.5)$ $\,\,$  & $1.624(18)$ $\,\,$ $1.674(18)$ $\,\,$ $1.722(19)$ $\,\,$  \\ 
B55.32	& $502.3(5.0)$ $\,\,$ $532.1(5.3)$ $\,\,$ $560.4(5.5)$ $\,\,$  & $1.637(17)$ $\,\,$ $1.685(18)$ $\,\,$ $1.733(18)$ $\,\,$  \\ 
B75.32	& $523.1(5.1)$ $\,\,$ $552.0(5.4)$ $\,\,$ $579.6(5.7)$ $\,\,$  & $1.642(17)$ $\,\,$ $1.692(17)$ $\,\,$ $1.740(18)$ $\,\,$  \\ 
B85.24	& $535.9(5.6)$ $\,\,$ $564.1(5.9)$ $\,\,$ $591.2(6.1)$ $\,\,$  & $1.651(14)$ $\,\,$ $1.701(14)$ $\,\,$ $1.750(15)$ $\,\,$  \\ 
\hline \\[-2.0ex] 
D15.48	& $442.9(4.6)$ $\,\,$ $477.8(4.9)$ $\,\,$ $510.3(5.3)$ $\,\,$  & $1.580(16)$ $\,\,$ $1.632(16)$ $\,\,$ $1.684(17)$ $\,\,$  \\ 
D20.48	& $449.8(4.9)$ $\,\,$ $484.2(5.2)$ $\,\,$ $516.4(5.6)$ $\,\,$  & $1.588(13)$ $\,\,$ $1.640(14)$ $\,\,$ $1.691(14)$ $\,\,$  \\ 
D30.48	& $464.0(5.0)$ $\,\,$ $497.5(5.3)$ $\,\,$ $529.1(5.6)$ $\,\,$  & $1.582(17)$ $\,\,$ $1.636(18)$ $\,\,$ $1.688(19)$ $\,\,$  \\ 
\end{tabular}


==> isoQCD/Data/TeX/ensembles/masses/pi_N_Delta.tex <==
\begin{tabular}{l|c|c|c}
Ensemble & $M_\pi$ (MeV) & $M_N$ (GeV) & $M_\Delta$ (GeV) \\ 
\hline \\[-2.0ex] 
A100.24	& $434.2(4.3)$ & $1.304(13)$ & $1.482(12)$\\ 
A30.32	& $242.5(2.6)$ & $1.114(19)$ & $1.309(21)$\\ 
A40.20	& $288.1(3.8)$ & $1.220(21)$ & $1.402(25)$\\ 
A40.24	& $283.4(3.7)$ & $1.170(23)$ & $1.319(32)$\\ 
A40.32	& $277.0(3.0)$ & $1.147(12)$ & $1.333(17)$\\ 
A40.40	& $278.1(3.0)$ & $1.122(13)$ & $1.333(18)$\\ 
A40.48	& $276.7(3.0)$ & $1.150(12)$ & $1.313(16)$\\ 
A50.32	& $307.7(2.9)$ & $1.166(17)$ & $1.353(14)$\\ 
A60.24	& $339.7(3.7)$ & $1.201(20)$ & $1.396(29)$\\ 
A80.24	& $388.8(4.2)$ & $1.255(17)$ & $1.429(20)$\\ 
\hline \\[-2.0ex] 
B25.32	& $235.0(2.5)$ & $1.117(20)$ & $1.330(24)$\\ 
B35.32	& $273.5(2.9)$ & $1.131(16)$ & $1.358(22)$\\ 
B55.32	& $339.0(3.5)$ & $1.200(14)$ & $1.409(17)$\\ 
B75.32	& $394.7(3.8)$ & $1.239(15)$ & $1.440(15)$\\ 
B85.24	& $423.2(4.5)$ & $1.274(13)$ & $1.456(20)$\\ 
\hline \\[-2.0ex] 
D15.48	& $204.4(2.0)$ & $1.048(16)$ & $1.312(31)$\\ 
D20.48	& $231.8(2.3)$ & $1.092(15)$ & $1.346(32)$\\ 
D30.48	& $282.5(3.1)$ & $1.094(14)$ & $1.316(24)$\\ 
\end{tabular}


==> isoQCD/Data/TeX/ensembles/masses/pi_N_Delta_K1_Omega1.tex <==
\begin{tabular}{l|c|c|c|c|c}
Ensemble & $M_\pi$ (MeV) & $M_N$ (GeV) & $M_\Delta$ (GeV) &$M_{K_1}$ (MeV) & $M_{\Omega_1}$ (GeV) \\ 
\hline \\[-2.0ex] 
A100.24	& $434.2(4.3)$ & $1.304(13)$ & $1.482(12)$ & $547.3(5.5)$ & $1.673(15)$\\ 
A30.32	& $242.5(2.6)$ & $1.114(19)$ & $1.309(21)$ & $484.4(5.2)$ & $1.623(15)$\\ 
A40.20	& $288.1(3.8)$ & $1.220(21)$ & $1.402(25)$ & $500.7(5.7)$ & $1.663(25)$\\ 
A40.24	& $283.4(3.7)$ & $1.170(23)$ & $1.319(32)$ & $496.9(5.4)$ & $1.647(21)$\\ 
A40.32	& $277.0(3.0)$ & $1.147(12)$ & $1.333(17)$ & $491.5(5.0)$ & $1.628(17)$\\ 
A40.40	& $278.1(3.0)$ & $1.122(13)$ & $1.333(18)$ & $490.4(5.1)$ & $1.635(16)$\\ 
A40.48	& $276.7(3.0)$ & $1.150(12)$ & $1.313(16)$ & $491.2(5.2)$ & $1.638(19)$\\ 
A50.32	& $307.7(2.9)$ & $1.166(17)$ & $1.353(14)$ & $500.3(5.0)$ & $1.635(17)$\\ 
A60.24	& $339.7(3.7)$ & $1.201(20)$ & $1.396(29)$ & $512.3(5.5)$ & $1.639(24)$\\ 
A80.24	& $388.8(4.2)$ & $1.255(17)$ & $1.429(20)$ & $528.1(5.6)$ & $1.647(19)$\\ 
\hline \\[-2.0ex] 
B25.32	& $235.0(2.5)$ & $1.117(20)$ & $1.330(24)$ & $473.9(4.8)$ & $1.616(15)$\\ 
B35.32	& $273.5(2.9)$ & $1.131(16)$ & $1.358(22)$ & $483.0(4.9)$ & $1.624(18)$\\ 
B55.32	& $339.0(3.5)$ & $1.200(14)$ & $1.409(17)$ & $502.3(5.0)$ & $1.637(17)$\\ 
B75.32	& $394.7(3.8)$ & $1.239(15)$ & $1.440(15)$ & $523.1(5.1)$ & $1.642(17)$\\ 
B85.24	& $423.2(4.5)$ & $1.274(13)$ & $1.456(20)$ & $535.9(5.6)$ & $1.651(14)$\\ 
\hline \\[-2.0ex] 
D15.48	& $204.4(2.0)$ & $1.048(16)$ & $1.312(31)$ & $442.9(4.6)$ & $1.580(16)$\\ 
D20.48	& $231.8(2.3)$ & $1.092(15)$ & $1.346(32)$ & $449.8(4.9)$ & $1.588(13)$\\ 
D30.48	& $282.5(3.1)$ & $1.094(14)$ & $1.316(24)$ & $464.0(5.0)$ & $1.582(17)$\\ 
\end{tabular}

